Proactive Message Passing on Memory Factor Networks

We introduce a new type of graphical model that we call a "memory factor network" (MFN). We show how to use MFNs to model the structure inherent in many types of data sets. We also introduce an associated message-passing style algorithm called "proactive message passing"' (PMP) that performs inference on MFNs. PMP comes with convergence guarantees and is efficient in comparison to competing algorithms such as variants of belief propagation. We specialize MFNs and PMP to a number of distinct types of data (discrete, continuous, labelled) and inference problems (interpolation, hypothesis testing), provide examples, and discuss approaches for efficient implementation.

==> MT.tex <==
\section{Memory tables}
\label{sec.MT}

In this section we describe a version of a memory factor network
wherein each factor node takes the form of a ``memory table.''  A
memory table is simply a database of exemplars, each exemplar
depicting a valid configuration of the variables that neighbor the
factor in question. Memory factors that are memory tables are
trivial to train.  If we are given a number of exemplars from which to
learn local structure we simply store $x^a = \{x_i : i \in \hood{a}\}$
for each exemplar.  We think of each of these stored snapshots as a
``memory.''  

Formally, the memory table corresponding to factor $a$ is a database
of $L_a$ (generally) distinct memories $\{\mem{a}{l} : l \in [L_a]\}$.
Each memory $\mem{a}{l}$ is a vector of length $|\hood{a}|$, the $j$th
element of which is $\memInd{a}{l}{j}$.  Each element of this vector
corresponds to a particular variable that neighbors factor $a$.  If
$\memInd{a}{l}{j}$ refers to variable $x_k$ ($k$ is the $j$th element
of $\hood{a}$) , then $\memInd{a}{l}{j} \in \mathcal{X}_k$.  The
memory table corresponding to factor $a$ is perhaps most conveniently
thought of as an $L_a \times |\hood{a}|$ array of variable values.

Note that evidence factors can be thought of as a special case of
memory table factors in which there is a single dynamic ``memory''
($L_a = 1$) corresponding to the current state of the evidence.

The selection cost $\selCost{a}(\cdot)$ we use in PMP for memory table
$a$ restricts the factor's opinions (and thus votes) to memories that
are in the table.  This is accomplished by using selection cost
\begin{equation*}
\selCost{a}(\bar{o}) = \left\{ \begin{array}{ccc} 0 & \mbox{if} & \exists \ l \in [L_a] \ \mbox{s.t.} \ \bar{o} = \mem{a}{l}\\ \infty & \mbox{otherwise.} \end{array} \right.
\end{equation*}
This choice simplifies~(\ref{alg.costComp}) in the PMP algorithm.  The
outside $\arg \min$ over $\bar{o}$ simply restricts the optimization
to opinions that exist in memory table $a$, for which the selection cost is zero.

The confidence $\kappa(a)$ of a memory table factor $a$ is the
difference in total cost (as specified by~(\ref{alg.costComp}))
between the best and second-best distinct sets of opinions
corresponding to its memories. Intuitively, a memory table factor has
high confidence that its choice of memory is correct, even if that
memory is costly, if the next best alternative is much
worse. Therefore it makes sense for this factor to cast its votes now
and allow other less confident factors to react to its decision.



==> autoencoders.tex <==
\section{Autoencoders}
\label{sec.autoencoders}

Another particular form of learned structure we can utilize for memory factors is
the \emph{autoencoder}. In particular we consider linear autoencoders, which
take the form of transformations from hidden variables $z \in \mathcal{Z}^p$
to visible variables $y \in \mathcal{Y}^n$ for appropriate variable spaces
$\mathcal{Z} \subseteq \mathbb{C}$ and $\mathcal{Y} \subseteq \mathbb{C}$. Thus the
autoencoder itself is a matrix $W \in \mathbb{C}^{n \times p}$. These
autoencoders may be learned from data by  a variety of methods,
e.g.~nonnegative matrix factorization. For our purposes we  simply consider
them to encode information about some of the variables in the  network.
Because we do not apply any sparsity assumptions to $W$ or to the hidden
variable $z$, we generally assume $p < n$ and thus the autoencoder provides a
low-dimensional representation of the visible variables, which are constrained
to lie in some low dimensional subspace of $\mathcal{Y}^n$.

In the context of a MFN, let us suppose a particular memory  factor $a$
represents an autoencoder, which maps $p_a$ hidden variables $z \in
\mathcal{Z}_a^{p_a}$  to $n_a$ visible variables $y \in \mathcal{Y}_a^{n_a}$.
We require the set of neighboring  variables $\hood{a}$ to include all visible
variables represented by the  autoencoder, as the variables represented in the
MFN are presumed to be those of  interest in the problem. We may also allow
$\hood{a}$ to include the hidden variables  represented by the autoencoder,
but this is not required. Generally hidden variables will be present in the
network if and only if there are connections between hidden variables at
different memory factors in the network. This may be possible if the learning
method supplies some semantic meaning for hidden variables that could be
shared across different parts of the problem. In our examples, however, hidden
variables will not be shared, and thus going forward we assume $\hood{a}$ is
precisely the set of visible variables for the autoencoder $a$, and thus $n_a
= |\hood{a}|$ and $\mathcal{Y}_a = \mathcal{X}_i$ for $i \in \hood{a}$. Note
that this restricts all variables in $\hood{a}$ to have the same alphabet, a
restriction that could be lifted by allowing autoencoders to have visible
variables in different alphabets. Such autoencoders are possible, but we do
not consider them here.

\subsection{Selection cost and opinion updates}

To specify the autoencoder as a memory factor, we must give the selection cost
$\selCost{a}$ for votes from the autoencoder. We use the cost
\begin{equation}\label{eq.AE-selcost}
\selCost{a}(\voteVec{a}) = 
\begin{cases} 0 & \exists z \in \mathcal{Z}_a^{p_a} \st \voteVec{a} = W_az \\
			\infty & \text{ otherwise.}
\end{cases}
\end{equation}
This cost simply requires the vote $\voteVec{a}$ to be in the subspace defined
by the autoencoder, and allows the hidden variables to take on any value in
their domain. Because the selection cost is either zero or infinite, we can
replace it in the opinion update optimization with a feasibility constraint,
so the problem becomes
\begin{equation*}
  \opinVec{a}  = \argmin_{\bar{o},z \st \bar{o} = W_a z} \left\{ \min_{x^a}
  \sum_{i \in \hood{a}} \left[ \locCost{i}(x_i, \bar{o}_i) \wt{i}{a} + 
    \sum_{b \in (\hood{i}\backslash\{a\}) \backslash \abstSet} \locCost{i}(x_i, \vote{i}{b}) \wt{i}{b}
  \right]\right\}
\end{equation*}
where $z$ is taken over $\mathcal{Z}_a^{p_a}$. While this is a reasonable
constraint for a variety of variable types, our examples make use of the case
where $\bar{o}$ and $z$ are both complex or both real. Using the notation of
Section \ref{sec.varTypes}, for real variables with quadratic cost the problem is is
\begin{align}\label{eq.AE-local-prob}
\argmin \quad \sum_{i \in \hood{a}}&\frac{\wt{i}{a}(\wtSum{i}-\wt{i}{a})}{\wtSum{i}}\left(\bar{o}_i - \bar{x}_i \right)^2 \\
\subjectto \quad\quad \bar{o} &= W_az. \notag
\end{align}
This convex quadratic program is small and straightforward to solve with a
second-order cone solver like SCS. Note that linear restrictions can be included in the
alphabet $\mathcal{X}_i$ without altering the nature of this problem. One
example is the case $\mathcal{X}_i= \mathbb{R}_+$ in which the problem becomes
\begin{align*}\label{eq.AE-nonneg-local-prob}
\argmin \quad \sum_{i \in \hood{a}}&\frac{\wt{i}{a}(\wtSum{i}-\wt{i}{a})}{\wtSum{i}}\left(\bar{o}_i - \bar{x}_i \right)^2 \\
\subjectto \quad\quad \bar{o} &= W_az \\
\bar{o}, z &\ge 0.
\end{align*}
We can also extend the problem to complex variables with cost $\locCost{i}(u,v) = |u - v|^2$.

